Improving Pointwise Mutual Information (PMI) by Incorporating Significant Co-occurrence

We design a new co-occurrence based word association measure by incorporating the concept of significant cooccurrence in the popular word association measure Pointwise Mutual Information (PMI). By extensive experiments with a large number of publicly available datasets we show that the newly introduced measure performs better than other co-occurrence based measures and despite being resource-light, compares well with the best known resource-heavy distributional similarity and knowledge based word association measures. We investigate the source of this performance improvement and find that of the two types of significant co-occurrence - corpus-level and document-level, the concept of corpus level significance combined with the use of document counts in place of word counts is responsible for all the performance gains observed. The concept of document level significance is not helpful for PMI adaptation.

==> tex/conclusions.tex <==
\section{Conclusions}
\label{sec:conclusions}

In this paper, we show that the concept of  Document-level significant co-occurrence 
is useful, even outside the context of CSR measure where it was
introduced. Our extensive experiments show that a
newly introduced measure SCI-z (SCI adapted for  Document-level
significant co-occurrence) performs better than the traditional word
association measures as well as the CSR.


\begin{comment}
\section*{Acknowledgments}
\revision{
This work was supported in part by the Ministry of Human Resources Development, 
Government of India and 
by the Tata Research Development and Design Center (TRDDC). 
\revisiontwo{We thank Mr. Justin Washtell (University of Leeds) for providing us with various datasets.}
}
\end{comment}


==> tex/discussion.tex <==
\section{Discussion}

Threshold span needs discussion. Essentially we say that, it is reasonable to believe that all
occurrences with span less than the threshold value can plausibly be motivated, while all
occurrences with span greater than the threshold span are probably arbitrary. This notion applies to
all co-occurrence based measures, not just the CSR



==> tex/figures.tex <==

\begin{figure}
  \begin{center}
    \begin{tabular}{cc}
	\resizebox{80mm}{!}{\includegraphics[angle=-90]{gnuplot/sim/simExpiryTimeDeltaS}} &
	\resizebox{80mm}{!}{\includegraphics[angle=-90]{gnuplot/sim/simExpiryTimeEffectW}} \\
    \end{tabular}
    \caption{Effect of span threshold on correlation of significance ratio (CSR) with human judgement}
    \label{expiryTimeDeltaFigs}
  \end{center}
\end{figure}

\begin{figure}
  \begin{center}
     \addtolength{\tabcolsep}{-9pt}
    \begin{tabular}{ccc}
	\resizebox{60mm}{!}{\includegraphics[angle=-90]{gnuplot/sim/simScatterPlot}} &
	\resizebox{60mm}{!}{\includegraphics[angle=-90]{gnuplot/sim/simScatterPlot1}} &
      	\resizebox{60mm}{!}{\includegraphics[angle=-90]{gnuplot/sim/simScatterPlot2}} \\	
    \end{tabular}
    \caption{Variation in correlation of various co-occurrence measures with human judgement}
    \label{expiryTimeFigs}
  \end{center}
\end{figure}


%\begin{figure}[h]
%  \centering
%    \includegraphics[width=0.5\textwidth]{gnuplot/esslli/esslliExpiryTimeEffectS}
%  \caption{esslliExpiryTimeEffectS.png}
%\end{figure}
%
%\begin{figure}[h]
%  \centering
%    \includegraphics[width=0.5\textwidth]{gnuplot/esslli/esslliExpiryTimeEffectW}
%  \caption{esslliExpiryTimeEffectW.png}
%\end{figure}
%
%\begin{figure}[h]
%  \centering
%    \includegraphics[width=0.5\textwidth]{gnuplot/rel/relExpiryTimeEffectS}
%  \caption{relExpiryTimeEffectS}
%\end{figure}
%
%\begin{figure}[h]
%  \centering
%    \includegraphics[width=0.5\textwidth]{gnuplot/rel/relExpiryTimeEffectW}
%  \caption{relExpiryTimeEffectW}
%\end{figure}
\begin{comment}
\begin{figure}
  \begin{center}
    \begin{tabular}{cc}
	\resizebox{80mm}{!}{\includegraphics[angle=-90]{gnuplot/sim/simExpiryTimeDeltaW}} &
	\resizebox{80mm}{!}{\includegraphics[angle=-90]{gnuplot/sim/simExpiryTimeDeltaS}} \\
    \end{tabular}
    \caption{Effect of expiry time on correlation of Significance Ratio with Human Judgement}
    \label{expiryTimeDeltaFigs}
  \end{center}
\end{figure}


\begin{figure}
  \begin{center}
    \begin{tabular}{cc}
	\resizebox{80mm}{!}{\includegraphics[angle=-90]{gnuplot/sim/simExpiryTimeEffectW}} &
      	\resizebox{80mm}{!}{\includegraphics[angle=-90]{gnuplot/sim/simExpiryTimeEffectS}} \\
    \end{tabular}
    \caption{Effect of expiry time on correlation of different measures with Human Judgement}
    \label{expiryTimeFigs}
  \end{center}
\end{figure}

\end{comment}


==> tex/tables.tex <==
\begin{table}
\small \addtolength{\tabcolsep}{-3pt}
\begin{tabular}{|l | c c c c |}
\hline
Measure	&	Similarity	&	Relatedness	&	WordSim353	&	ESSLLI	\\ 
\hline
CSR & 0.66 & 0.62 & 0.60 & 0.44 \\
PMI & 0.74 & 0.69 & 0.70 & 0.34 \\
LLR & 0.57 & 0.55 & 0.51 & 0.38 \\
Dice & 0.67 & 0.59 & 0.60 & 0.37 \\
Ochiai & 0.69 & 0.64 & 0.63 & 0.46 \\
Jaccard & 0.67 & 0.59 & 0.60 & 0.37 \\
TTest & 0.50 & 0.49 & 0.44 & 0.34 \\
ChiSquare & 0.69 & 0.64 & 0.63 & 0.46 \\
SCI & 0.44 & 0.38 & 0.37 & 0.46 \\
CWCD & 0.64 & 0.53 & 0.56 & 0.36 \\
MCD & 0.69 & 0.57 & 0.62 & 0.37 \\
\hline
\end{tabular}
\caption{ \small Best correlation for each measure}
\label{BestPerformanceTable}
\end{table}


\begin{table}
\tiny \addtolength{\tabcolsep}{-3pt}
\begin{tabular}{|l | l l l l l l l l l|}
\hline
& \begin{sideways}CSR (2s)\end{sideways} & \begin{sideways}PMI (15w)\end{sideways} & \begin{sideways}LLR (5w)\end{sideways} & \begin{sideways}Dice (10w)\end{sideways} & \begin{sideways}Ochiai (1s)\end{sideways} & \begin{sideways}TTest (5w)\end{sideways} & \begin{sideways}SCI (5w)\end{sideways} & \begin{sideways}CWCD (10w)\end{sideways} & \begin{sideways}MCD (doclen)\end{sideways} \\
\hline
CSR (2s) & 1.00 & 0.72 & 0.90 & 0.91 & 0.93 & 0.86 & 0.77 & 0.70 & 0.85 \\
PMI (15w) & 0.72 & 1.00 & 0.62 & 0.71 & 0.73 & 0.50 & 0.48 & 0.85 & 0.78 \\
LLR (5w) & 0.90 & 0.62 & 1.00 & 0.95 & 0.94 & 0.98 & 0.85 & 0.66 & 0.74 \\
Dice (10w) & 0.91 & 0.71 & 0.95 & 1.00 & 0.97 & 0.91 & 0.80 & 0.76 & 0.79 \\
Ochiai (1s) & 0.93 & 0.73 & 0.94 & 0.97 & 1.00 & 0.91 & 0.80 & 0.72 & 0.84 \\
TTest (5w) & 0.86 & 0.50 & 0.98 & 0.91 & 0.91 & 1.00 & 0.85 & 0.57 & 0.66 \\
SCI (5w) & 0.77 & 0.48 & 0.85 & 0.80 & 0.80 & 0.85 & 1.00 & 0.73 & 0.58 \\
CWCD (10w) & 0.70 & 0.85 & 0.66 & 0.76 & 0.72 & 0.57 & 0.73 & 1.00 & 0.68 \\
MCD (doclen) & 0.85 & 0.78 & 0.74 & 0.79 & 0.84 & 0.66 & 0.58 & 0.68 & 1.00 \\
\hline
\end{tabular}
\caption{ \small Correlation Matrix for Similarity Dataset}
\label{SimCorrlMatrix}
\end{table}


\begin{table}
\tiny \addtolength{\tabcolsep}{-3pt}
\begin{tabular}{|l | l l l l l l l l l|}
\hline
& \begin{sideways}CSR (5s)\end{sideways} & \begin{sideways}PMI (15w)\end{sideways} & \begin{sideways}LLR (5w)\end{sideways} & \begin{sideways}Dice (15w)\end{sideways} & \begin{sideways}Ochiai (20w)\end{sideways} & \begin{sideways}TTest (5w)\end{sideways} & \begin{sideways}SCI (5w)\end{sideways} & \begin{sideways}CWCD (5w)\end{sideways} & \begin{sideways}MCD (doclen)\end{sideways}
 \\
\hline
CSR (5s) & 1.00 & 0.63 & 0.88 & 0.85 & 0.93 & 0.86 & 0.71 & 0.55 & 0.86\\
PMI (15w) & 0.63 & 1.00 & 0.58 & 0.65 & 0.70 & 0.46 & 0.38 & 0.76 & 0.68\\
LLR (5w) & 0.88 & 0.58 & 1.00 & 0.92 & 0.95 & 0.99 & 0.78 & 0.62 & 0.78\\
Dice (15w) & 0.85 & 0.65 & 0.92 & 1.00 & 0.96 & 0.90 & 0.72 & 0.67 & 0.77\\
Ochiai (20w) & 0.93 & 0.70 & 0.95 & 0.96 & 1.00 & 0.92 & 0.74 & 0.65 & 0.85\\
TTest (5w) & 0.86 & 0.46 & 0.99 & 0.90 & 0.92 & 1.00 & 0.79 & 0.54 & 0.73\\
SCI (5w) & 0.71 & 0.38 & 0.78 & 0.72 & 0.74 & 0.79 & 1.00 & 0.71 & 0.6\\
CWCD (5w) & 0.55 & 0.76 & 0.62 & 0.67 & 0.65 & 0.54 & 0.71 & 1.00 & 0.58\\
MCD (doclen) & 0.86 & 0.68 & 0.78 & 0.77 & 0.85 & 0.73 & 0.60 & 0.58 & 1.00\\
\hline
\end{tabular}
\caption{ \small Correlation Matrix for Relatedness Dataset}
\label{RelCorrlMatrix}
\end{table}

\begin{table}
\tiny \addtolength{\tabcolsep}{-3pt}
\begin{tabular}{| l | l l l l l l l l l|}
\hline
& \begin{sideways}CSR (5s)\end{sideways} & \begin{sideways}PMI (15w)\end{sideways} & \begin{sideways}LLR (5w)\end{sideways} & \begin{sideways}Dice (15w)\end{sideways} & \begin{sideways}Ochiai (20w)\end{sideways} & \begin{sideways}TTest (5w)\end{sideways} & \begin{sideways}SCI (5w)\end{sideways} & \begin{sideways}CWCD (10w)\end{sideways} & \begin{sideways}MCD (doclen)\end{sideways} \\
\hline
CSR (5s) & 1.00 & 0.62 & 0.88 & 0.85 & 0.92 & 0.85 & 0.71 & 0.55 & 0.83  \\
PMI (15w) & 0.62 & 1.00 & 0.54 & 0.64 & 0.70 & 0.41 & 0.37 & 0.80 & 0.76  \\
LLR (5w) & 0.88 & 0.54 & 1.00 & 0.92 & 0.94 & 0.98 & 0.79 & 0.55 & 0.74  \\
Dice (15w) & 0.85 & 0.64 & 0.92 & 1.00 & 0.96 & 0.89 & 0.73 & 0.67 & 0.77  \\
Ochiai (20w) & 0.92 & 0.70 & 0.94 & 0.96 & 1.00 & 0.90 & 0.75 & 0.65 & 0.84  \\
TTest (5w) & 0.85 & 0.41 & 0.98 & 0.89 & 0.90 & 1.00 & 0.80 & 0.46 & 0.67  \\
SCI (5w) & 0.71 & 0.37 & 0.79 & 0.73 & 0.75 & 0.80 & 1.00 & 0.68 & 0.57  \\
CWCD (10w) & 0.55 & 0.80 & 0.55 & 0.67 & 0.65 & 0.46 & 0.68 & 1.00 & 0.62  \\
MCD (doclen) & 0.83 & 0.76 & 0.74 & 0.77 & 0.84 & 0.67 & 0.57 & 0.62 & 1.00  \\
\hline
\end{tabular}
\caption{ \small Correlation Matrix for WordSim353 Dataset}
\label{Wordsim353CorrlMatrix}
\end{table}

\begin{table}
\tiny \addtolength{\tabcolsep}{-3pt}
\begin{tabular}{|l | l l l l l l l l l|}
\hline
& \begin{sideways}CSR (5s)\end{sideways} & \begin{sideways}PMI (15w)\end{sideways} & \begin{sideways}LLR (5w)\end{sideways} & \begin{sideways}Dice (20w)\end{sideways} & \begin{sideways}Ochiai (25w)\end{sideways} & \begin{sideways}TTest (5w)\end{sideways} & \begin{sideways}SCI (15w)\end{sideways} & \begin{sideways}CWCD (15w)\end{sideways} & \begin{sideways}MCD (doclen)\end{sideways} \\
\hline
CSR (5s) & 1.00 & 0.42 & 0.86 & 0.79 & 0.88 & 0.84 & 0.69 & 0.40 & 0.59 \\
PMI (15w) & 0.42 & 1.00 & 0.33 & 0.52 & 0.56 & 0.19 & 0.21 & 0.95 & 0.77 \\
LLR (5w) & 0.86 & 0.33 & 1.00 & 0.87 & 0.90 & 0.98 & 0.64 & 0.34 & 0.53 \\
Dice (20w) & 0.79 & 0.52 & 0.87 & 1.00 & 0.95 & 0.82 & 0.42 & 0.48 & 0.53 \\
Ochiai (25w) & 0.88 & 0.56 & 0.90 & 0.95 & 1.00 & 0.85 & 0.62 & 0.53 & 0.62 \\
TTest (5w) & 0.84 & 0.19 & 0.98 & 0.82 & 0.85 & 1.00 & 0.65 & 0.20 & 0.41 \\
SCI (15w) & 0.69 & 0.21 & 0.64 & 0.42 & 0.62 & 0.65 & 1.00 & 0.32 & 0.41 \\
CWCD (15w) & 0.40 & 0.95 & 0.34 & 0.48 & 0.53 & 0.20 & 0.32 & 1.00 & 0.77 \\
MCD (doclen) & 0.59 & 0.77 & 0.53 & 0.53 & 0.62 & 0.41 & 0.41 & 0.77 & 1.00 \\
\hline
\end{tabular}
\caption{ \small Correlation Matrix for ESSLLI Dataset}
\label{EsslliCorrlMatrix}
\end{table}



%\begin{table}
%\small\addtolength{\tabcolsep}{-3pt}
%\begin{tabular}{l c c c}\hline   
%Method    & Overall & Similarity & Relatedness \\ \hline
%CSR & 0.62 & 0.66 & 0.63\\
%WN30g & 0.66 & 0.72 & 0.56 \\
%BoW & 0.65 & 0.70 & 0.62 \\
%CW & 0.60  & 0.77  & 0.46  \\ \hline
%\end{tabular}
%\caption{ \small Comparison with previous work for Similarity, Relatedness and WordSim353 }
%\label{relsimTable}
%\end{table}


\begin{table}
\tiny \addtolength{\tabcolsep}{-3pt}
\begin{tabular}{p{3cm} l l}   
 \hline
Method & Source & Correlation\\
\hline
CSR (5s) & Wikipedia (April 2008) & 0.60 \\
WN30g & XXX & 0.66 \\
BoW & XXX & 0.65 \\ 
CW & XXX & 0.60  \\ 
Strube and Ponzetto, 2006 & Wikipedia & 0.19-0.48 \\
Jarmasz, 2003 &  WordNet & 0.33-0.35 \\
Jarmasz, 2003 & Roget's & 0.55 \\
Hughes and Ramage, 2007 & WordNet & 0.55 \\
Finkelstein et al., 2002 & Web corpus, WN & 0.56 \\
%(Gabrilovich and Markovitch, 2007) & ODP & 0.65 \\
Gabrilovich and Markovitch, 2007 (reimplemented in [REF]) & Wikipedia& 0.75 \\
\hline
\end{tabular}
\caption{ \small Comparison with previous work for WordSim353 }
\label{prevWorkTable}
\end{table}



\begin{table}
\small 
\begin{tabular}{|l| l| l |l| l| l|}   
 \hline
Method & Formula & \begin{sideways}Symmetry \end{sideways} & \begin{sideways}Null Addition \end{sideways}& \begin{sideways}Inversion \end{sideways}& \begin{sideways}Homogenity \end{sideways}\\
\hline
CSR &  & Y & Y & N & N\\ \hline 
LLR & $N\left(\sum_{i,j} p(i,j)log\frac{p(i,j)}{p(i)p(j)}\right)$ & Y & N & Y & Y \\ \hline
PMI & $\frac{p(x,y)}{p(x)p(y)}$ & Y & Y & N & Y \\ \hline
SCI & $\frac{p(x)p(y)}{p(x)\sqrt{p(y)}}$ & N & Y  & N  & Y\\ \hline
CWCD & $\frac{\hat{f}(x,y)}{p(x)}\frac{1/max\left(p(x),p(y)\right)}{M}$ & N & Y  & N & Y\\ \hline
MCD &  $1/M $  & X & X & X & X\\ \hline
Pearson's $\chi^2$ test & $\sum_{i,j} \frac{\left(\hat{f}(i,j)-E\hat{f}(i,j)\right)^2}{E\hat{f}(i,j)}$ & Y & N & Y & Y\\ \hline
T-test & $\frac{\hat{f}(x,y)-E\hat{f}(x,y)}{\sqrt{\hat{f}(x,y)\left(1-\frac{\hat{f}(x,y)}{N}\right)}}$ & Y & Y & N & Y\\ \hline
Dice & $\frac{2\hat{f}(x,y)}{f(x)+f(y)}$ & Y & Y & N & Y\\ \hline
Ochiai & $\frac{\hat{f}(x,y)}{\sqrt{f(x)f(y)}}$ & Y & Y & N & Y\\ \hline
Jaccard & $\frac{\hat{f}(x,y)}{f(x)+f(y)-\hat{f}(x,y)}$ & Y & Y & N & Y \\ \hline
\end{tabular}
\small
Terminology: \\
\scalebox{0.8}{%
\begin{tabular}{l l }   
$\hat{f}(x,y)$ & Constrained word pair frequency\\
$N$ & Total number of tokens in the corpus \\
$p(x,y)$ & $\hat{f}(x,y)/N $\\
$M$ & Harmonic mean of the spans of $\hat{f}(x,y)$ occurrences\\
$E\hat{f}(i,j)$ & Expected value of f(i,j): $\left(p(i)/N\right) \times \left(p(j)/N\right) \times N$ \\
$f(x)$ & frequency of $x$ in the corpus \\
\hline
\end{tabular}
}
\caption{ \small Properties of methods }
\label{methods}
\end{table}

\clearpage

